Simple Questions Generate Named Entity Recognition Datasets

Recent named entity recognition (NER) models often rely on human-annotated datasets, requiring the significant engagement of professional knowledge on the target domain and entities. This research introduces an ask-to-generate approach that automatically generates NER datasets by asking questions in simple natural language to an open-domain question answering system (e.g., "Which disease?"). Despite using fewer in-domain resources, our models, solely trained on the generated datasets, largely outperform strong low-resource models by an average F1 score of 19.4 for six popular NER benchmarks. Furthermore, our models provide competitive performance with rich-resource models that additionally leverage in-domain dictionaries provided by domain experts. In few-shot NER, we outperform the previous best model by an F1 score of 5.2 on three benchmarks and achieve new state-of-the-art performance.

==> sections/complexity.tex <==

\section{Complexity Analysis}
\input{tables/complexity}
From automatic dataset generation to model training, \ours~is a very efficient framework. 
In \Cref{tab:complexity}, we show the time taken for each step in \ours~for CoNLL-2003.
Dataset generation steps (Step 1, 2, and 3) mostly take about 10 minutes in total while the self-training step (Step~4) take about 30 minutes.

==> sections/missing.tex <==

\section{Analysis}

This section presents several results in \Cref{sec:analysis} that were omitted due to space limitations.

%
%\input{figures/top_k_all}
%\paragraph{Effect of the number of sentences}
%\Cref{fig:top_k_all} shows performance changes with different numbers of sentences for each NER benchmark.

%
%\input{tables/rule_ablation}
%\paragraph{Effect of normalization rules}
%\Cref{tab:rule_ablation} shows the results of applying various normalization rules on NCBI-disease and BC5CDR.

%
\input{tables/complexity}
\paragraph{Complexity analysis}
\Cref{tab:complexity} shows the time taken for each step in the entire \ours~framework, which were omitted due to space limitations.



==> sections/top_k.tex <==
\section{Effect of the number of sentences}
\input{figures/top_k_all}
\Cref{fig:top_k_all} shows how performance changes when increasing the total number of retrieved sentences for each dataset.
The performance tends to increase at first but decrease after the highest points, which indicates that simply increasing the number of entities does not help.
We suspect that the number of phrases with incorrect types might increase, causing the performance degradation.

==> tables/results_biomedical.tex <==
\begin{table*}[t]
\centering
\begin{adjustbox}{max width = 0.99\textwidth}

\begin{tabular}{lcrrrrrrrrr}
\toprule
\multirow{2}{*}{\textbf{Model}} & \textbf{In-domain} & \multicolumn{3}{c}{\textbf{NCBI-disease}} & \multicolumn{3}{c}{\textbf{BC5CDR}} & \multicolumn{3}{c}{\textbf{CHEMDNER}} \\
 & \textbf{sent. / dict. / label} &  \multicolumn{1}{c}{\textbf{\precision}} & \multicolumn{1}{c}{\textbf{\recall}} & \multicolumn{1}{c}{\textbf{\fscore}} & \multicolumn{1}{c}{\textbf{\precision}} & \multicolumn{1}{c}{\textbf{\recall}} & \multicolumn{1}{c}{\textbf{\fscore}} & \multicolumn{1}{c}{\textbf{\precision}} & \multicolumn{1}{c}{\textbf{\recall}} & \multicolumn{1}{c}{\textbf{\fscore}}  \\
\midrule
\multicolumn{10}{l}{\textit{Rich-resource setting (w/ in-domain dict. or label)}} \\
\midrule
\biobert~\cite{lee2020biobert} & \cmark~/~\xmarkspace/~\cmark & 86.6\smallspace & 90.5\smallspace & 88.5\smallspace & 86.7\smallspace & 90.5\smallspace & 88.6\smallspace & 91.4\smallspace & 91.1\smallspace & 91.2\smallspace \\
\bond~\cite{liang2020bond} & \cmark~/~\cmark~/~\xmark & 87.5\smallspace & 60.3\smallspace & 71.4\smallspace & 81.0\smallspace & 80.3\smallspace & 80.6\smallspace & -\smallspace & -\smallspace & -\smallspace \\
%Dictionary & \cmarkspace / \cmarkspace / \xmarkspace & 79.13 & 52.92 & 63.42 & 86.32 & 59.94 & 70.75 & - & - & - \\
\midrule
\multicolumn{10}{l}{\textit{Low- or zero-resource setting}} \\
\midrule
Seed Entities & \cmark~/$^{\,}$\partiallyused$^{\,}$/~\xmark & \textbf{88.8}\outperformbond & 10.7\smallspace & 19.1\smallspace & {\textbf{95.7}}\outperformbond & 3.6\smallspace & 6.9\smallspace & \textbf{93.7} & 12.2\smallspace & 21.5\smallspace \\
Neural Tagger & \cmark~/$^{\,}$\partiallyused$^{\,}$/~\xmark & 75.2\smallspace & 24.9\smallspace & 37.4\smallspace & {93.1}\outperformbond & 9.7\smallspace & 17.6\smallspace & 74.8\smallspace & 21.6\smallspace & 33.5\smallspace  \\
Self-training & \cmark~/$^{\,}$\partiallyused$^{\,}$/~\xmark & 67.5\smallspace & 35.1\smallspace & 46.2\smallspace & 73.3\smallspace & 12.7\smallspace & 21.6\smallspace & 41.2\smallspace & 44.7\smallspace & 42.9\smallspace \\
\tallor$^\dagger$~\cite{li-etal-2021-weakly} & \cmark~/$^{\,}$\partiallyused$^{\,}$/~\xmark & -\smallspace & -\smallspace & -\smallspace & 66.5\smallspace & 66.9\smallspace & 66.7\smallspace & 63.0\smallspace & 60.2\smallspace & 61.6\smallspace \\
\tallor~\cite{li-etal-2021-weakly} & \cmark~/$^{\,}$\partiallyused$^{\,}$/~\xmark & 61.5\smallspace & 34.7\smallspace & 44.3\smallspace & 65.6\smallspace & 56.8\smallspace & 61.9\smallspace & 61.6\smallspace & 51.5\smallspace & 56.1\smallspace \\
%\cq~(\textbf{ours}) & \xmarkstar / \xmarkspace / \xmarkstar & 67.44 & 54.17 & 60.08 & 65.84 & \textbf{78.38} & 71.57 & 38.65 & 67.83 & 49.24 \\
\ours~(\textbf{ours}) & \xmarkspace/~\xmarkspace/~\xmark & {78.6}\smallspace & {\textbf{72.7}}\outperformbond & {\textbf{75.5}}\outperformbond & 71.4\smallspace & \textbf{77.1}\smallspace & \textbf{74.2}\smallspace & {58.6}\smallspace & \textbf{68.8}\smallspace & \textbf{63.2}\smallspace \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
The performance of baseline models and our models on three benchmarks in the biomedical domain.
The description of the table is the same as in Table \ref{tab:main_general}.
%\jinhyuk{apply same changes as in Table 4}
}
\label{tab:main_biomedical}
\end{table*}


%% 

\begin{comment}

\begin{table*}[]
\centering
\footnotesize
\begin{adjustbox}{max width = 0.99\textwidth}

\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{NCBI-disease} & \multicolumn{3}{c}{BC5CDR} & \multicolumn{3}{c}{CHEMDNER} \\
 &  \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F}  \\
\midrule
\multicolumn{10}{l}{\textbf{Supervised}} \\
BioBERT & 86.55 & 90.52 & 88.49 & 86.70 & 90.48 & 88.55 & 91.40 & 91.08 & 91.24 \\
\midrule
\multicolumn{10}{l}{\textbf{Distantly supervised}} \\
Dictionary & 79.13 & 52.92 & 63.42 & 86.32 & 59.94 & 70.75 & - & - & - \\
BOND & 87.46 & 60.28 & 71.37 & 80.98 & 80.30 & 80.64 & - & - & - \\
\midrule
\multicolumn{10}{l}{\textbf{Baseline models}} \\
Seed Entities & \outperformbond{88.79} & 10.73 & 19.14 & \outperformbond{95.66} & 3.60 & 6.94 & 93.72 & 12.17 & 21.54 \\
Neural Tagger & 75.16 & 24.90 & 37.40 & \outperformbond{93.07} & 9.73 & 17.61 & 74.84 & 21.59 & 33.51  \\
Self-training &  &  &  &  &  & &  &  &  \\
TaLLoR$^\dagger$ & - & - & - & 66.53 & 66.94 & 66.73 & 63.01 & 60.18 & 61.56 \\
TaLLoR & 61.48 & 34.67 & 44.33 & 65.58 & 56.82 & 61.90 & 61.57 & 51.48 & 56.07 \\
\midrule
\multicolumn{10}{l}{\textbf{Ours (Wikipedia)}} \\
GeNER-\textsc{dq} & \textbf{78.61} & \textbf{72.69} & \textbf{75.53} & 78.72 & 65.82 & \textbf{71.69} & \textbf{66.70} & \textbf{80.61} & \textbf{73.00} \\
GeNER-\textsc{cq} & 67.44 & 54.17 & 60.08 & 65.84 & \textbf{78.38} & 71.57 & 38.65 & 67.83 & 49.24 \\
\multicolumn{10}{l}{\textbf{- w/o self-training}} \\
GeNER-\textsc{dq} & 62.57 & 56.77 & 59.53 & \textbf{80.19} & 52.07 & 63.14 & 58.20 & 57.63 & 57.92  \\
GeNER-\textsc{cq} & 43.51 & 52.40 & 47.54 & 69.17 & 74.09 & 71.55 & 37.64 & 59.65 & 46.15   \\
\midrule
\multicolumn{10}{l}{\textbf{Ours (PubMed)}} \\
GeNER-\textsc{dq} & \\
GeNER-\textsc{cq} & \\
\multicolumn{10}{l}{\textbf{- w/o self-training}} \\
GeNER-\textsc{dq} & \\
GeNER-\textsc{cq} & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{}
\label{tab:my-table}
\end{table*}

\end{comment}

==> tables/results_crossner.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{max width = 0.99\textwidth}
\begin{tabular}{lccccccc}
\toprule
Method & \begin{tabular}[c]{@{}l@{}}Target\\ Unlabeled\end{tabular} & \multicolumn{1}{c}{Politics} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Natural\\ Science\end{tabular}} & \multicolumn{1}{c}{Music} & Literature & \begin{tabular}[c]{@{}l@{}}Artificial\\ Intelligence\end{tabular} & Average \\
\midrule
\multicolumn{8}{l}{\textbf{Supervised}} \\
Fine-tune only$^\dagger$  & - & 66.56 & 63.73 & 66.59 & 59.95 & 50.37 & 61.44 \\
Pre-train + Fine-tune$^\dagger$  & - & 68.71 & 64.94 & 68.30 & 63.63 & 58.88 & 64.89 \\
DAPT$^\dagger$ & \cmark & 69.37 & 66.68 & 72.05 & 65.15 & 61.48 & 66.95 \\
\midrule
\multicolumn{8}{l}{\textbf{Baseline Models}} \\
Seed entities & - & \begin{tabular}[c]{@{}c@{}}25.80\\ (57.80/16.60)\end{tabular} & \begin{tabular}[c]{@{}c@{}}27.37\\ (68.70/17.09)\end{tabular} & \begin{tabular}[c]{@{}c@{}}25.39\\ (66.27/15.70)\end{tabular} & \begin{tabular}[c]{@{}c@{}}21.56\\ (60.32/13.12)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}39.59\\ (72.62/27.21)\end{tabular} & \begin{tabular}[c]{@{}c@{}}27.94\\ (65.14/17.94)\end{tabular}  \\
CGExpand & \cmark &  &  &  &  \\
Self-training & \cmark &  &  &  &  \\
TaLLoR & \cmark &  &  &  &  \\
\midrule
\multicolumn{8}{l}{\textbf{Ours}} \\
GeNER-\textsc{dq} &  -  &  &  &  &  \\
\quad w/o Self-training &  -  &  &  & & \begin{tabular}[c]{@{}c@{}}36.63\\ (49.41/29.11)\end{tabular} &  & \\
GeNER-\textsc{cq} &  -  &  &  & \begin{tabular}[c]{@{}c@{}}33.65\\ (25.93/47.89)\end{tabular} & \begin{tabular}[c]{@{}c@{}}38.71\\ (29.24/57.25)\end{tabular} & \begin{tabular}[c]{@{}c@{}}26.70\\ (30.88/23.52)\end{tabular} &  \\
\quad w/o Self-training &  -  &  &  & \begin{tabular}[c]{@{}c@{}}30.11\\ (24.90/38.08)\end{tabular} & \begin{tabular}[c]{@{}c@{}}30.83\\ (25.47/39.05)\end{tabular} & \begin{tabular}[c]{@{}c@{}}31.61\\ (39.93/26.17)\end{tabular} & \\
GeNER-\textsc{mix} & - &  &  &  &  \\
\quad w/o Self-training &  -  &  &  &  &  &  & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
\cmark and - indicate that models use or do not use training resources that require human effort, respectively.
$\triangle$ indicates that models use only the entities in the target labeled data, not the whole sentence.
}
\label{tab:my-table}
\end{table*}


